NatCat: Weakly Supervised Text Classification with Naturally Annotated Resources

We describe NatCat, a large-scale resource for text classification constructed from three data sources: Wikipedia, Stack Exchange, and Reddit. NatCat consists of document-category pairs derived from manual curation that occurs naturally within online communities. To demonstrate its usefulness, we build general purpose text classifiers by training on NatCat and evaluate them on a suite of 11 text classification tasks (CatEval), reporting large improvements compared to prior work. We benchmark different modeling choices and resource combinations and show how tasks benefit from particular NatCat data sources.

==> intro-old.tex <==
\section{Introduction}

\zewei{\natcat is a knowledge base automatically constructed from three data sources: Wikipedia, Stackoverflow, and Reddit. With rich world knowledge, \natcat is proved to be a useful resource for zero-shot text classifications. }\kevin{I like the idea of focusing the intro on NatCat rather than dataless text classification, but I don't think we should necessarily start out by saying that NatCat is a knowledge base, because I think we would get pushback on that. But we could build up to that claim by the end of the introduction and ultimately say something like ``We can also view NatCat as a simple knowledge base extracted from these resources; it has one type of relation corresponding to the topical text classification relationship.''}

% \kevin{In both this intro and the related work, some of the papers we cite describe what they do in ways other than ``weakly-supervised'', and it would be good to be more faithful to how they describe their work. That is, some of these papers are actually much closer to a zero-shot setting than our work. Our work is more weakly-supervised than zero-shot, but that doesn't mean that we should describe the related work as weakly-supervised. E.g., Yogatama actually do something like zero-shot text classification, and other papers do as well. So the replacement of ``zero-shot'' with ``weak supervision'' should only be made when describing our models/methods/paper, not necessarily when describing other researchers' work, for which other terms are more accurate. This could be an annoying change, but I think it's important and is relevant to the question of why our method is better than others (i.e., because it's weakly-supervised instead of being true zero-shot classification).}

The goal of weakly supervised (aka. ``dataless'') text classification is to classify documents without a priori knowledge of target labels. It has the obvious advantage over standard supervised approaches of being label-agnostic: 
a single model can be used for different labels without re-training. 
But the performance of weakly supervised classifiers is often significantly behind that of supervised models, limiting their usefulness.

Previous works focus on restricted domains such as medical text 
\cite{mullenbach2018explainable,rios2018few}, leverage additional information
such as semantic knowledge graphs \cite{zhang-etal-2019-integrating},
or carefully exploit weak supervision such as class keywords 
\cite{meng2019weakly} to achieve satisfactory performance. 
However, they suffer from a limited scope, a need for nontrivial extra 
supervision that is difficult to obtain in a large amount, 
and rather complicated methodologies.

Instead, we consider a more practical setting: is there a readily 
available resource that we can use to obtain a simple model that can 
robustly handle a wide range of open-domain text classification tasks? 
Our primary contribution is a new dataset, \natcat, 
% and a set of effective weakly supervised models 
% that serve as strong 
that can be used to train strong text classification models. 
% baselines on this dataset for future studies. 
\natcat is constructed from naturally annotated text from a variety of online resources. 
In particular, we use Wikipedia, Stack Exchange, and Reddit as the source of document-category pairs. 

% Wikipedia articles manually tagged with over a million fine-grained categories. 
We train models on \natcat to compute similarity between any document-category pair.
As a result, they can be used as off-the-shelf classifiers that produce interpretable and 
relevant Wikipedia topics for any document. They can also be effortlessly ported to a specific topic classification task 
and categorize documents under the labels of the task. 
Table~\ref{tab:example1} illustrates the use of our model on a document from \agnews. 


\begin{table}[t]
\setlength{\tabcolsep}{2pt}
\small
\begin{center}
\begin{tabular}{cp{13.3cm}}
 \multirow{3}{*}{\bf Text} & Israeli ambassador calls peace conference idea `counterproductive'. A broad international peace conference that has reportedly been suggested by Egypt could be ``counterproductive'' and shouldn't be discussed until after ...\\
\addlinespace
 \multirow{1}{*}{\bf \natcat} &  \emph{invasions}, \emph{diplomats}, \emph{peace}, \emph{diplomacy}, \emph{environmentalism}, \emph{Egypt}, \emph{patriotism} ... \\
\addlinespace
\multirow{1}{*}{\bf AGNews} & \textbf{\emph{international}}, \emph{sports}, \emph{science technology}, \emph{business} \\
\hline
\end{tabular}
\end{center}
%\vspace{-0.2cm}
\caption{\label{tab:example1} An instance of weakly supervised topic classification from \agnews, the highest scoring categories from \natcat, and ranked \agnews categories (true class in bold).}
\end{table}

To evaluate, we propose \cateval, a standardized benchmark for evaluating weakly supervised text classification with a choice of datasets, label descriptions for each dataset, and baseline results. 
\cateval comprises a diverse choice of 11 text classification tasks inlcuding both topic-related and sentiment related labels, and contains both single and multi-label classification tasks. 


We show that training on \natcat leads to strong baselines for future work in weakly supervised text classification, and study the impact of \natcat  data domain and pretrained model choice on particular tasks in \cateval. 

Our work builds on previous approaches to weakly supervised text classification and is also
significantly different in various ways. 
Unlike generic representations such as Explicit Semantic Analysis (ESA)
\cite{chang-dataless,gabrilovich-esa}, 
we explicitly introduce a surrogate training task for neural models
(scoring document-category pairs) that faithfully approximates
the end goal of text classification.
Our scale is much larger than the small dataset-specific experiments in \cite{yogatama-generative-discrimitive}, and we do not require additional supervision
at test time such as seed words as in topic modeling approaches \cite{li2016effective,chen2015dataless}. 

%downstream training data lead to different -trained models outperform all existing weakly supervised text classifiers over the \cateval tasks. 
% the classic ESA approach and also 
% recent models such as GloVe~\cite{pennington-glove}, ELMo~\cite{peters-elmo-2018}, and BERT~\cite{devlin2018bert}.
We analyze the gap between weakly supervised and supervised models 
and show that the mistakes of our models are reasonable and humanlike. 
